Network Alignment by Discrete Ollivier-Ricci Flow

In this paper, we consider the problem of approximately aligning/matching two graphs. Given two graphs $G_{1}=(V_{1},E_{1})$ and $G_{2}=(V_{2},E_{2})$, the objective is to map nodes $u, v \in G_1$ to nodes $u',v'\in G_2$ such that when $u, v$ have an edge in $G_1$, very likely their corresponding nodes $u', v'$ in $G_2$ are connected as well. This problem with subgraph isomorphism as a special case has extra challenges when we consider matching complex networks exhibiting the small world phenomena. In this work, we propose to use `Ricci flow metric', to define the distance between two nodes in a network. This is then used to define similarity of a pair of nodes in two networks respectively, which is the crucial step of network alignment. %computed by discrete graph curvatures and graph Ricci flows. Specifically, the Ricci curvature of an edge describes intuitively how well the local neighborhood is connected. The graph Ricci flow uniformizes discrete Ricci curvature and induces a Ricci flow metric that is insensitive to node/edge insertions and deletions. With the new metric, we can map a node in $G_1$ to a node in $G_2$ whose distance vector to only a few preselected landmarks is the most similar. The robustness of the graph metric makes it outperform other methods when tested on various complex graph models and real world network data sets (Emails, Internet, and protein interaction networks)\footnote{The source code of computing Ricci curvature and Ricci flow metric are available: https://github.com/saibalmars/GraphRicciCurvature}.

==> future_works.tex <==
\chapter{Future Works on Discrete Graph Ricci Flow} % (fold)
\label{cha:future_works}

\section{Introduction on Ricci Flow} 

Ricci flow was introduced by Richard Hamilton for Riemannian manifolds of any dimension in 1982. A surface Ricci flow is the process to deform the Riemannian metric of the surface. The deformation is proportional to the Gaussian curvature, such that the curvature evolves like the heat diffusion. At the limit the surface has uniform curvature everywhere. 
 
Here we are the first to consider Ricci flow in the graph setting. For a given graph $G=(V,E)$, let the edge weight of edge $xy \in E$ to be $d(x,y)$, and Ricci curvature to be $\kappa(x,y)$, then we take:
$$ d_{i+1}(x,y)=d_{i}(x,y)-\eps \cdot \kappa_{i}(x,y) \cdot d_{i}(x,y).$$
At each iteration, we recompute the Ricci curvature on each edge based on the current edge weight, then update the edge weight until the Ricci curvature on all edges converge to the same value.

As the network curvature is uniform everywhere the edges are provided with different weights. Edges of initially positive curvature are getting shorter while edges of initially negative curvature get longer. This correlates well with the properties of strong/weak ties in a social network setting. Further, the uniformization of curvature properly `stretches out' the network in a meaningful way. 

For future work, we plan to apply the ricci flow metric for the following purpose 
Graph Matching: Given two graphs G1 and G2 with approximately the same graph topology, we wish to find the correspondence of vertices – each vertex v in G1 is mapped to a vertex f(v) in G2 such that whenever u, v are connected in G1, f(u), f(v) are likely to be connected in G2 as well.
Label Propagation: Given a graph and a partial labeling of the vertices, we would like to propagate the labels to discover the hidden attributes of others. This is related to the problem of creating a metric between nodes in the network that captures the similarity of the vertices.
Graph Comparison and Classification: Given two graphs, we would like to come up with a topological descriptor for a graph so that we can evaluate the similarity of two graphs for graph comparison and classification.


\section{Graph Matching} 
The problem of graph matching is closely related to the classical problem of \emph{graph isomorphism}, in which we test whether or not two graphs have \emph{exactly} the same topology under a proper correspondence. 
A related setting is to consider two graphs $G_1$ and $G_2$ that differ, but only by a small amount. And the goal is to find correspondences for most of vertices such that two nodes have an edge in $G_1$ and very likely their corresponding vertices have an edge in $G_2$. 

Graph isomorphism or graph matching problem has numerous applications ranging from database schema matching, protein interaction alignment, ontology matching, and pattern recognition. 
%[3] S. Melnik, H. Garcia-Molina, and E. Rahm, “Similarity flood- ing: A versatile graph matching algorithm and its application to schema matching,” in Proc. of the 18th Intl. Conf. on Data Engineering. IEEE Computer Society, 2002, p. 117.
%[2] R. Singh, J. Xu, and B. Berger, “Pairwise global alignment of protein interaction networks by matching neighborhood topology,” in Proc. of the 11th Annual Intl. Conf. on Research in Computational Molecular Biology (RECOMB), ser. LNCS, vol. 4453. Springer, 2007, pp. 16–31.
%[4] O. Sˇva ́b, “Exploiting patterns in ontology mapping,” in Proc. of the 6th Intl. Semantic Web Conf., ser. LNCS, K. A. et al., Ed., vol. 4825. Berlin, Heidelberg: Springer, November 2007, pp. 950–954.
%[5] D. Conte, P. P. Foggia, C. Sansone, and M. Vento, “Thirty years of graph matching in pattern recognition,” Intl. J. of Pattern Recognition and Artificial Intelligence, vol. 18, no. 3, pp. 265–298, May 2004.
%[8] R. Singh, J. Xu, and B. Berger, “Global alignment of multiple protein interaction networks with application to functional orthology detection,” PNAS, vol. 105, no. 35, pp. 12763– 12 768, September 2008.
Here we mainly focus on complex networks that appear in real world setting. 
Consider the Internet backbone graphs captured at two different points in time, we wish to match the vertices of the two graphs in order to understand how the network evolved over time. Or, consider two social network topologies on the same group of users. It is likely that when two users are connected by a social tie in one network (say LinkedIn), they are also connected in the other network (say Facebook). A good matching of the two networks can be useful for many applications such as feature prediction, link prediction, anomaly detection, and possibly de-anonymization.

The problem of graph isomorphism has been heavily studied. The subgraph isomorphism problem, i.e., testing whether one graph is the subgraph of the other, is known to be NP-complete. But it is unclear if the graph isomorphism is in NP or not. Polynomial isomorphism algorithms have been developed for special kinds of graphs (e.g. for trees~\cite{Aho:1974:DAC:578775}, for planar graphs~\cite{Hopcroft:1974:LTA:800119.803896}, for bounded valence graphs~\cite{10.1109/SFCS.1980.24}). 
%A. V. Aho, J. E. Hopcroft and J. D. Ullman, The Design and Analysis of Computer Algorithms (Addison Wesley, 1974).
%J.E.HopcroftandJ.Wong,Lineartimealgorithmforisomorphismofplanargraphs, in Proc. 6th Annual ACM Symp. Theory of Computing, 1974, pp. 172–184.
%E. M. Luks, Isomorphism of graphs of bounded valence can be tested in polynomial time, J. Comput. Syst. Sci. 25 (1982) 42–65.
For general graphs, the most recent breakthrough by L\'{a}szl\'{o} Babai~\cite{DBLP:journals/corr/Babai15} shows an algorithm with improved running time in quasi-polynomial time $O(\exp{((\log n)^{O(1)})})$, where $n$ is the number of vertices of the graphs. Other ideas use tree-based search, optimization, and spectral methods. In practice, the fastest heuristics for graph isomorphism is the algorithm called \textsc{Nauty}~\cite{McKay1981,McKay2014}, which uses the automorphism group of each of the input graphs. 
%Unfortunately, this algorithm  cannot work for noisy graph matching.
%B. D. McKay, Practical graph isomorphism, Congressus Numerantium 30 (1981) 45–87.
For approximate graph isomorphism (or noisy graph matching), some algorithms used for exact matching (such as \textsc{Nauty}) fail. But many other ideas that use graph edit distance, tree-based matching, and statistical methods can often apply. See the survey for references~\cite{ConteFSV04,Yan:2016:SSR:2911996.2912035,Emmert-Streib:2016:FYG:2906473.2906531}.

%Chien-Chun: VF2 citation as follows might help.

%\cite{Cordella:2004fa}
%Luigi P. Cordella, Pasquale Foggia, Carlo Sansone, Mario Vento, “A (Sub)Graph Isomorphism Algorithm for Matching Large Graphs”, IEEE Transactions on Pattern Analysis and Machine Intelligence, vol. 26, no. 10, pp. 1367-1372, Oct., 2004. http://ieeexplore.ieee.org/iel5/34/29305/01323804.pdf

%\cite{Cordella:2001vr}
%L. P. Cordella, P. Foggia, C. Sansone, M. Vento, “An Improved Algorithm for Matching Large Graphs”, 3rd IAPR-TC15 Workshop on Graph-based Representations in Pattern Recognition, Cuen, pp. 149-159, 2001. http://amalfi.dis.unina.it/graph/db/papers/vf-algorithm.pdf

%\paragraph{Our Method.} 
Since the graph curvatures capture inherently the structures of the graphs, in both local and global manners, we propose to use graph curvatures and Ricci flows to tackle noisy or inexact graph matching. 

%To better understand the challenge, let us consider the problem of matching two noisy graphs. 
We first look at the following instance to get the intuition and understand the challenge in handling real world complex networks. Suppose we have $k$ landmarks with known correspondence for a small constant $k$. In many settings there are special vertices that can be identified and matched. If no such prior landmarks are given, we can always enumerate for a subset of $k$ vertices. To find the correspondences of the other vertices, one idea is to represent each vertex in the graph by its relative position to the set of landmarks, and match two vertices if their positions in the networks are similar. Suppose the landmarks are denoted by $\{\ell_i, i=1, 2, \cdots, k\}$, we can define a landmark based coordinate vector for each node $v\in G_j$ as $[d_j(v, \ell_1), d_j(v, \ell_2), \cdots, d_j(v, \ell_k)]$, where $d_j(v, \ell_i)$ denotes the network distance from $v$ to $\ell_i$. Now if a node $u\in G_1$ has a coordinate vector very similar to the coordinate vector of a node $v \in G_2$, we can match $u$ and $v$. While this makes sense in general, immediately we realize that using hop count as network distance suffers from terribly low resolution. Most real world complex networks have small world property -- the diameter is a small integer say $6$. Thus any distance value in the distance vector is an integer of 1 to $6$. Many nodes may have the same distance vector unless we use a fairly large number of landmarks. Thus we cannot directly use the hop count value as the lack of distinguishing capabilities. 

Other ideas in generating coordinates for vertices in a graph is to find an embedding of the graph and use the embedding to provide an edge weight to define the network distance between two nodes. One may use spring embedding~\cite{Tutte:1963tz} or the spectral embedding~\cite{Luxburg:2007:TSC:1288822.1288832}. 
For example, in spring embedding (aka Tutte embedding or barycentric embedding), we fix the coordinates of a subset of nodes (say the landmarks) and each other node updates its coordinates at the center of mass of its neighbors until convergence.  Alternatively, we can also try the spectral embedding~\cite{Luxburg:2007:TSC:1288822.1288832} which uses the eigenvectors for the smallest $h$ non-zero eigenvalues of the graph Laplacian $L=D-A$ (where $D$ is the diagonal degree matrix and $A$ is the adjacency matrix) to generate the node coordinates in $\reals^h$. 
These embedding methods work great with isomorphic graphs -- as they are deterministic methods, but are unstable when edges/nodes are inserted and removed. Graph spectrum can change drastically when nodes/edges are inserted/removed, which affects the results for classification of graphs~\cite{Wilson:2008:SGS:1379924.1380381}. The metric by Ricci flow turns out to be much more stable. See Figure~\ref{fig:graph_matching} for preliminary results on comparing two graphs.

\begin{figure}[htbp]
	\centering
	\vspace*{-2mm}
	\subfigure[$G$ v.s. $G$.]{
		\label{fig:gnp-0}
		\includegraphics[width=0.6\columnwidth]{figure/gnp-remove0node}}
		%\vspace{-6mm}
	\hspace{0mm}
	\subfigure[$G$ v.s. $G_{-1}$. $G_{-1}$ is $G$ with randomly removed $1$ node and $9$ corresponding edges.]{
		\label{fig:gnp-1}
		\includegraphics[width=0.6\columnwidth]{figure/gnp-remove1Node}}
		% \vspace{-2mm}
	\hspace{0mm}
	\subfigure[$G$ v.s. $G_{-10}$. $G_{-10}$ is $G$ with randomly removed $10$ nodes and $88$ corresponding edges.]{
		\label{fig:gnp-10}
		\includegraphics[width=0.6\columnwidth]{figure/gnp-remove10Node}}
		\vspace{-2mm}

	\caption{\small A graph matching comparison result on a Erdös-Rényi Graph $G$ with node removals over different edge weight metrics. Here $G$ has $1000$ nodes and $4979$ edges. While the recovery accuracy drops drastically with spectral and spring embedding, the Ricci flow metric remains stable.}
	\vspace{-2mm}
	\label{fig:graph_matching} %% label for entire figure
		
\end{figure}

% \paragraph{Proposed Tasks.}
% In this project we plan to thoroughly study the graph Ricci flow and the application in graph matching. Our directions are:
% \benum
% \item Study the stability of the metric under graph dynamics for noisy graph matching;
% %\item Study the produced metric and properties for representing the latent social space, and finally
% \item Speed up the computation of discrete Ricci curvature and graph Ricci flow on large data.
% \eenum

\section{Graph Comparison and Clustering}

In this problem we consider comparing two graphs as well as classifying graphs into different families. This can be formulated into two problems:
\bitem
\item Define a similarity measure between two graphs that may not be labeled. 
\item Classify a family of input graphs into clusters such that those in the same cluster have similar structures or are likely generated from the same models.  
\eitem

% \begin{wrapfigure}{r}{76mm}
\begin{figure}[thbp]
	\centering
		% \vspace{-8mm}
	% \hspace*{-7mm}
	\includegraphics[width=0.65\columnwidth]{figure/MDS_ricci_model_rm}
	% \vspace{-11mm}
	\caption{\small{The figure shows the clustering of graphs generated from different models. We calculate the earth mover distance on the curvature distribution between graphs. We use Multi-Dimensional Scaling to generate the embedding. Here all the model graphs have $1000$ nodes and around $4000$ edges. It can be seen that graphs generated from the same model graph (with the same color) are tightly clustered. %The same type of model are clearly form a cluster in thes measure space.
	}}
 % \vspace{-6mm}
	\label{fig:mds}
\end{figure}
% \end{wrapfigure}


Again here the problem is related to graph isomorphism -- that if two graphs are isomorphic their similarity should be $1$ and shall be put in the same cluster. Graph isomorphism is however too strict for most applications. Alternatively, one may use graph edit distance, in which we count the number of operations that are necessary to transform $G_1$ into $G_2$. One can assign costs to different types of operations (edge/node insertion/deletion, modification of labels). A third approach is to come up with feature vectors (topological descriptors) and then use existing tools for comparing these feature vectors.  Probably the most popular approach is to use graph kernels~\cite{Vishwanathan:2010:GK:1756006.1859891}, which compares substructures of graphs that are computable in polynomial time. 
The first kernel method, called the convolution kernel~\cite{haussler99convolution}, compare all pairs of decompositions of two structured objects. What is used more often is based on random walks~\cite{Kashima03marginalizedkernels,Gartner03ongraph}. Improvements of the random graph walk kernel were later introduced in~\cite{NIPS2006_836,Mahe:2004:EMG:1015330.1015446,Borgwardt:2005:SKG:1106326.1106333}: label enrichment, tottering prevention, and replacing random walks by paths. 
%Kashima et al., ICML 2003, Gaertner et al., COLT 2003
%Fast computation of random walk graph kernels (Vishwanathan et al., NIPS 2006)
%Label enrichment and preventing tottering (Mahe et al., ICML 2004) 
%Graph kernels based on shortest paths (B. and Kriegel, ICDM 2005)
Recent methods adopted various graph substructures to compute kernels and combine them with edit distance, graphical models, group theory, etc~\cite{Frohlich:2005:OAK:1102351.1102380,Menchetti:2005:WDK:1102351.1102425,Neuhaus:2006:RWK:2090325.2090352,Ramon03expressivityversus,Horvath:2004:CPK:1014052.1014072,DBLP:conf/mlg/BorgwardtPVK07,Bach:2008:GKP:1390156.1390160,Kondor:2008:SSG:1390156.1390219}.
%Froehlich et al., ICML 2005
%Menchetti et al., ICML 2005
%Neuhaus and Bunke, 2006
%Ramon and Gaertner, 2004
%Horvath et al., KDD 2004
%B., Petri, et al., MLG 2007
%Combine graph kernels with graphical models (Bach, ICML 2008)
%Combine graph kernels with group theory (Kondor and B., ICML 2008)

%On the other hand, curvature and Ricci flow has been used a lot for comparing shapes and other geometric objects. 
%\jie{David, do you have a few sentences we can copy here together with references from your prior work?}

%\paragraph{Proposed Tasks.} 
Here we will explore the use of graph curvatures for comparing and clustering graphs, as curvature and Ricci flow has been used a lot for comparing shapes and other geometric objects. To start we first examine the distribution of graph curvatures or the edge weights generated by graph Ricci flow as a signature of a graph. One can then compare the signatures of two graphs to evaluate their similarities, for example, by using the earth mover distance to compute the difference between two distributions. Here we show some preliminary results of comparing graphs curvatures generated by different models in Figure~\ref{fig:mds}. It is clear to see that graphs from the same models are much closer to each other in this measure space. 


% As for our proposed work, we plan to thoroughly examine and explore the potential of this idea. The directions include:
% \bitem
% \item Evaluate the dependency of curvature distribution with respect to features of the graphs such as edge density, and parameter choices.
% \item In addition to the curvature distribution of the graph which is a global measure, we also examine the local curvature distribution and develop new graph kernels.
% \item Compare the results for using graph curvatures and edge weights produced by graph Ricci flow.
% \eitem

%----------------------------------------------------------------------------------------------------
 % \begin{wrapfigure}{r}{65mm}
\begin{figure}
\centering
% \vspace{-10mm}
\includegraphics[width=0.5\columnwidth]{figure/semantic-existence}
\caption{\small A semantic word graph centered at word ``existence'', sampled from Roget~\cite{batagelj2006pajek}. Here the edge length and thickness correlate to the Ricci flow weights, closer words imply closer word similarity.}
\label{fig:semantic}
% \vspace{-4mm}
\end{figure}
 % \end{wrapfigure}
%----------------------------------------------------------------------------------------------------


\section{Label Propagation}

In the problem of label propagation, we consider the situation when a network is partially labeled with attributes (e.g., age, profession, etc) and we wish to predict the labels of the rest of nodes. This is a type of semi-supervised learning in the literature. Intuitively we want data points that are similar to have the same label. In general learning problems the graph is constructed by using some similarity measure of the input data, and then keep the kNN graph (each node keeps edges to the $k$ nearest neighbor) or $\eps$NN graph (each node keeps the edges to all other nodes within distance $\eps$). In our setting the network is already given. But the neighborhood cannot be taken simply as the immediate neighbors as edges are not the same. 
%Strong ties connect people who regularly spend time with each other, while weak ties connect people who are just acquaintances. Strong and weak ties also exhibit structural differences -- one's close friends are more likely to be friends of each others and weak ties are more likely to connect people from different social communities. Label propagation and learning need to consider the tie strength which is often hard to directly measure. We need a more elaborative metric, ideally learned from the network structure itself. 
For label propagation and learning, previous work such as graph kernels~\cite{Vishwanathan:2010:GK:1756006.1859891}, DeepWalk~\cite{Perozzi:2014:DOL:2623330.2623732}, node2vec~\cite{Grover:2016:NSF:2939672.2939754} use controlled random walks to generate a neighborhood of each node. 

%\paragraph{Proposed Tasks.} 
We plan to adopt the metric generated by the Ricci flow for learning better weights on the edges. With the new weights, the neighbors of a node are those within shortest path distance of $r$ for a parameter $r$.  See Figure~\ref{fig:semantic} for an example on a semantic word network.  The words that are more related in meaning are indeed placed closer to each other. Again we plan to fully explore the potential of this idea. 

%It would be desirable to associate with each tie a weight measuring its strength, though it is challenging to do so as measuring tie strength either requires direct user input or additional information such as communication frequency. 




% chapter future_works (end)


==> related_work.tex <==
Graph pattern matching, also as known as subgraph isomorphism, graph simulations and so on, is a significant problem which highly related to problems such as graph database query, protein-protein interaction discovery and pattern recognition\cite{Fan:2013fm,EmmertStreib:2016ft}. In most of the problem setting, the given graphs are usually with node or edge attribute\cite{Khan:2013fu, Tong:2007ut}, and the pattern subgraphs are usually much smaller than given graph. Method of solving graph matching problem includes manipulate the matching over compressed graph\cite{Maccioni:2016vo}, spectral methods\cite{Singh:2008cp,Aflalo:2015hd}, random walks\cite{Tong:2007ut}, and optimal cost matching method\cite{Khan:2013fu}. 





==> ricci.tex <==
\section{Ricci Curvature on Graph} % (fold)

We first define the $\alpha$-Ricci Curvature on Graph based on Lin's definition~\cite{Lin:2011tt}.

Given a graph $G$ and a vertex $x\in G$ with degree $d_x$, let $\Gamma(x)=\lbrace x_1, x_2, \cdots ,x_m\rbrace$ denotes the sets of neighborhood of $x$.
For every vertex $x$ and $\alpha \in \left[ 0,1 \right]$, we define a probability measure $m_{x}^{\alpha}$ by it's neighbors as follows,
\begin{equation*}
m_{x}^{\alpha}(x_i)=
	\begin{cases}
	\alpha & \mbox{\ if } x_i = x\\
	\left( 1-\alpha\right)/d_x & \mbox{\ if } x_i \in \Gamma(x)\\
	0 & \mbox{\ otherwise }.
	\end{cases}
\end{equation*}

For any two distinct vertices $x, y \in G$, where $\overline{xy}$ is an edge in $G$, the $\alpha$-Ricci curvature of $\overline{xy}$ is defined to be
\begin{equation*}
\kappa_\alpha(x,y)= 1 - \dfrac{W(m_{x}^{\alpha}, m_{y}^{\alpha})}{d(x,y)},
\end{equation*}
where $W(m_{x}^{\alpha}, m_{y}^{\alpha})$ is the Wasserstein distance(earth mover distance) between two measures $m_{x}^{\alpha}$ and $m_{y}^{\alpha}$, and $d(x,y)$ is the weight on $\overline{xy}$.
For convenience, we fix $\alpha=0.5$ and write $\kappa^{\alpha}(x,y)$ as $\kappa(x,y)$ instead.

\section{Discrete Ricci Flow}

% Despite the rich literatures of discrete Ricci curvature on triangular mesh, the works on graph is fairly limited. In \cite{Ollivier:2010gg}, Ollivier proposed a ``discrete Ricci flow'' as follows,
% $$\frac{d}{dt}d(x,y)=-\kappa(x,y)d(x,y)$$

Ricci flow is a process that deforms the metric while the Ricci curvature evolves to be constant everywhere. To compute the discrete Ricci flow on undirected graph, we follow the hypothesis mentioned by Ollivier in \cite{Ollivier:2010gg}.

For a given graph $G=(V,E)$, let the edge weight of edge $\overline{xy} \in E$ to be $d(x,y)$, and Ricci curvature to be $\kappa(x,y)$, the Ricci flow of $G$ is evolved as follows,

$$ d_{i+1}(x,y)=d_{i}(x,y)-\epsilon \cdot \kappa_{i}(x,y) \cdot d_{i}(x,y) ,\quad \forall \overline{xy} \in E.$$

In our experiment, in order to avoid the ``blow up'' of metric, we rescale the metric so that the sum of edge weight remains constant. For each iteration, we recompute the Ricci curvature on each edge based on the current edge weight, then update and normalized the weight until the Ricci curvature on each edge converge to the same number $C$.
the detailed algorithm is as follows.

\begin{algorithm}
	\label{algo:ricci_flow}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}

    \Input{An undirected graph $G$.}
    \Output{A weighted graph $G$ with same Ricci curvature on every edge.}

	Normalize the edge weight $d_{i}(x,y) \leftarrow d_{i}(x,y) \cdot \frac{|E|}{\sum_{\overline{xy} \in E}d_{i}(x,y)}$
	
	Compute the Ricci curvature of $G$
	
	Update the edge weight by $d_{i+1}(x,y)\leftarrow d_{i}(x,y)-\epsilon \cdot \kappa_{i}(x,y) \cdot d_{i}(x,y)$
	
	Repeat $1-3$ until all $\kappa$ converge to the same value

    \caption{Discrete ricci flow}
\end{algorithm}

